Benchmarking 16-element quantum search algorithms on superconducting quantum processors

We present experimental results on running 4-qubit unstructured search on IBM quantum processors. Our best attempt attained probability of success around 24.5%. We try several algorithms and use the most recent developments in quantum search to reduce the number of entangling gates that are currently considered the main source of errors in quantum computations. Comparing theoretical expectations of an algorithm performance with the actual data, we explore the hardware limits, showing sharp, phase-transition-like degradation of performance on quantum processors. We conclude that it is extremely important to design hardware-aware algorithms and to include any other low level optimizations on NISQ devices.

==> MultipointOracle.tex <==
    
\section{Multipoint Oracle}
\label{section:multipoint}
    We now proceed to the unstructured search problem with multiple marked elements. As in previous sections we  assume that number of qubits in the input of the oracle is \( n \). 
    Let \(S\) be the set of elements marked by oracle \(O\) and let \(K=|S|>0\). For convenience we  mostly refer to the number  \(k = 1+\lceil \log_2{K} \rceil \). We begin our investigation with the assumption that \(k\) is known in advance and later proceed to consider the harder case of unknown \(k\).
    \subsection{Known Number of Marked Elements}    
    In this section we assume that value \(k\) is known. It is weaker assumption than knowing \(K\) but  it is sufficient for our purposes.
    
    We use algorithm from theorem \Cref{thm:main} as a subroutine in algorithms in this section.
    By \emph{\(\texttt{SinglePoint}(O,n)\)} we denote the algorithm from \Cref{thm:main} that solves unstructured search problem for oracle \(O\) which marks exactly one element and acts on \(n\) qubits.
    We want to reduce the problem of unstructured search with possibly many elements marked to the unstructured search with one marked element. To do this we construct a family of hash functions that allows us to effectively parametrize a subset of \( \{0,1\}^n \) which with high probability contains only one element from \(S\). This technique is nearly identical to reduction from SAT to UniqueSAT presented in \cite{valiant}. Next, we improve some aspects  of this reduction, so that methods of partial uncompute may be used to reduce the number of additional non-oracle basic gates.
    
    
    Let us recall that family \( U \) of hash functions from \(X \) to \( Y \), both being finite is called \emph{pairwise independent} if for every \(x \in X\) and every \(y \in Y\) we have:
    \[\PP_{h \in_R U}\paren*{h(x)=y} = \frac{1}{|Y|} \]
    and for every \(x_1, x_2  \in X\), \(x_1 \neq x_2\) and every \( y_1, y_2 \in Y \) we have:
    
    \[ \PP_{h \in_R U}\paren*{h(x_1)=y_1 \wedge h(x_2) = y_2} = \frac{1}{|Y|^2}. \] 
     
    We use the following formulation of results from \cite{valiant} that can be found in \cite[p9.10 (180)]{arora}.
    
    \begin{lem}[Valiant-Vazirani]\label{valian-vazirani}
    For any family of pairwise independent hash functions \(H
    \) from \(\{0,1\}^{n}\) to \(\{0,1\}^{k}\) and \(S \subset \{0,1\}^{n} \) such that \(2^{k-2}\leq |S| \leq 2^{k-1}\) we have that 
    \[ \PP_{h \in_R H}\paren*{ |\{x \in S : h(x)=0\}| =1 } \geq \frac{1}{8}\]
    \end{lem}

    
    A function \(h:\{0,1\}^m \rightarrow \{0,1\}^l\) is called \emph{affine} if we may represent it as \(h(x)=Ax+b\) for some \(A \in \{0,1\}^{l\times m} \) and \( b \in \{0,1\}^{l}\). All arithmetical operations are performed modulo \(2\). 
    
    The \emph{kernel} of the affine function \(h:\{0,1\}^m \rightarrow \{0,1\}^l\) of the form \(h(x)=Ax+b\) is defined as \( \ker{h} = h^{-1}(0) \). Whenever the kernel of the affine function \(h\) is not an empty set, we define the dimension of this kernel as \( \dim{\ker{h}} = \dim{\ker{A}} \). Where \( \ker{A} \) is the null space of the matrix \(A\).    
    
    Whenever function \(h\) is clear from the context we use \(d=\dim{\ker{h}} \) for brevity.
    Our choice of the family of hash functions is as follows. 
   
    \begin{ddef}
    Define a family of hash functions \( H_{n,k}\) as the set of all affine maps from \(\{0,1\}^{n}\) to \(\{0,1\}^{k}\):
    \[H_{n,k} = \{ h_{A,b} \colon A \in \{0,1\}^{k\times n}, b\in \{0,1\}^k, h_{A,b}(x)=Ax+b\}.\]  
    \end{ddef}
    
    The first mention of this family is in \cite{carter}, more detailed considerations can be found in \cite{toeplitz}.
    The following standard result will be of use to us.
    \begin{observation}[Folklore]\label{independence}
    The family \(H_{n,k}\) is pairwise independent.
    \end{observation}
    
    
    
    We would like to run algorithm \(\texttt{SinglePoint}\) on the set \(\ker{h} \). To do so we parametrize \(\ker{h}\) by some injection \( g: \{0,1\}^{\dim{\ker{h}}} \rightarrow \ker{h} \) and build a quantum oracle \(O_g\) defined as follows.
    
    \begin{ddef}\label{oprim}
    Given a quantum oracle \(O : (\mathbb{C}^2)^{\otimes n} \rightarrow (\mathbb{C}^2)^{\otimes n} \), and any function  \( g: \{0,1\}^{d} \rightarrow \{0,1\}^n \) we define \(g\)-\emph{restricted oracle} 
    \( O_g \) as: 
    \[O_g=D_g^{-1}(Id_d\otimes O) D_g, \] 
    where \(D_g\) is a unitary operator on \((\mathbb{C}^2)^{\otimes (d+n)} \) whose action on states \( \ket{i}\ket{0 \ldots 0} \) for \(i \in \{0,1\}^{d}\) is defined as 
    \[ D_g\ket{i}\ket{0 \ldots 0} = \ket{i}\ket{g(i)}. \]
    \end{ddef}
    
    \begin{observation}
    If oracle \(O\) admits uncomputable decomposition \((O_u, O_p)\) then for any function \(g : \{0,1\}^d \rightarrow \{0,1\}^n \) \(g\)-restricted oracle \(O_g\) admits an uncomputable decomposition \( ((Id_d\otimes O_u) D_g, Id_d\otimes O_p) \) 
    \end{observation}
    \begin{proof}
    It follows directly from definition
    \begin{align*}
    O_g &= D_g^{-1}(Id_d\otimes O) D_g=D_g^{-1}(Id_d\otimes O_{u}^{-1})(Id_d\otimes O_{p})(Id_d\otimes O_{u}) D_g\\
    &= ((Id_d\otimes O_{u}) D_g)^{-1} (Id_d\otimes O_{p}) ((Id_d\otimes O_{u}) D_g).
    \end{align*}
    
    \end{proof}
    
    \begin{lem}\label{dekorator}
    For an affine injective function \(g:\{0,1\}^{d} \rightarrow \ker{h} \) of the form \(g(x)=Cx+p\), where \(C=(c_{ij})\) we can construct \(D_g\) using basic quantum gates so that the number of gates that depend on \(i\)-th qubit of the first register is exactly equal to \(|\{j \colon c_{ij} = 1\}|\).
    \end{lem}
    \begin{proof}
    It is easy to see that \(D_g\) can be implemented using gates \(CX(f_i, s_j)\) where on \(f_i\) is the \(i\)-th qubit of the first register and \(s_j\) is  the \(j\)-th qubit of the second register for each \(i,j\) such that \(c_{ij}=1\) and using gates \(X(s_j)\) for all \(j\) such that \(p_j>0\). 
    
    \end{proof}
    
    Now we are ready to construct \(g\) which effectively parametrizes \(\ker{h}\).
    
    \begin{lem}\label{gauss-dziala}
    Given an affine function \(h:\{0,1\}^n \rightarrow \{0,1\}^k\) with \(\ker{h}\neq \emptyset\) we may construct in polynomial time 
    the injective function \( g: \{0,1\}^d \rightarrow \{0,1\}^n \) 
    of the form \( g(x)=Cx+p \) for some \( C \in \{0,1\}^{n\times d}, p \in \{0,1\}^n\)  and \(d =\dim{\ker{h}} \) such that
    \( \Ima{g}=\ker{h} \). 
    In addition to that we may choose \(C\) so that each of its columns has at most \(n-d+1\) ones.
    \end{lem}
    \begin{proof}
    We begin by obtaining an arbitrary affine parametrization of \(\ker{h}\). To this end fix some basis of \(\ker{A} \), arrange it as columns into the matrix \(C^{'}\) and any solution \(p\) to the equation \(Ax=-b\). All of this can be accomplished in polynomial time using Gaussian elimination \cite{gauss-elim}. 
    Setting \(f(x)=C^{'}x+p\) gives us the desired parametrization.
    
    
    To reduce number of ones in the matrix \(C^{'} \), we can change basis of domain of \(f \) by an invertible matrix \(Q \in \{0,1\}^{d\times d}\). 
    As function \(f\) is an injection, matrix \(C^{'}\) has \(d\) rows which are linearly independent and they form an invertible submatrix \(C^{''}\). By picking 
    \(Q=(C^{''})^{-1}\) we assure that for each column of matrix \(C^{'}Q\) at most one row among those \(d\) picked previously has one which is contained in this column. After these steps we end up with a function \(g\) of the form \(g(x)=C^{'}Qx+p\), where each column of \(C=C^{'}Q\) has at most \(n-d+1\) non-zero entries.
    \end{proof}

    
    
    
    
    As we  parametrize the kernel of random affine map we want to make sure that dimension of this kernel is not too big, as the number of oracle queries and the number of non-oracle basic gates used by \(\texttt{SinglePoint}\) depends exponentially on the dimension of the searched space.
    
    \begin{lem}\label{dimensionality}
    If \(k<n-2\) then \(  \PP_{h \in_R H_{n,k}}(\dim{\ker{h}} \geq n-k+2)  \leq \frac{1}{16} \). 
    \end{lem}
    \begin{proof}
    We prove the more general inequality \( \PP_{h \in_R H_{n,k}}(\dim{\ker{h}} \geq n-k+c)  \leq \frac{1}{2^{c^2}} \) for \(n>4\), \(k<n-2\) and any natural \(c \leq 2\).
    Set \(\delta = k-c \). If \(\delta < 0\) then the conclusion follows trivially. Otherwise
    the event \(\dim{\ker{h}} \leq n-k+x\)  is equivalent to \(  n-\delta = n-k+c  \leq \dim{\ker{h}} = \dim{\ker{A}} = n- \rank{A}\) so we conclude \(\rank{A}\leq \delta \), meaning that vector subspace spanned by rows of matrix \( A \) must have dimension at most \( \delta \). 
    
    As vectors that span subspace of dimension at most \(\delta\) are contained in some \(\delta\)-dimensional subspace of \(\{0,1\}^n\) we can consider the probability of all \(k\) vectors being contained in a particular \(\delta\)-dimensional subspace. Then we apply union bound by multiplying this probability by the number of \(\delta\)-dimensional subspaces.
    The probability of choosing all \( k \) vectors from a single \( \delta \)-dimensional space is \( \paren*{\frac{1}{2^{n-\delta}}}^k \), as \( \delta\)-dimensional space contains \(2^{\delta}\) elements and we choose those vectors independently from each other.
    Let us recall that a number of \( \delta \)-dimensional subspaces of \(n\) dimensional space over \(\mathbb{F}_2\) equals \(  \prod_{i=0}^{\delta-1} \frac{2^n-2^i}{2^{\delta}-2^i} \), this can be found in \cite{subspaces}.
     
    So using the union bound the probability that \(k\) vectors span at most \( \delta \)-dimensional subspace is bounded from above by:
    \begin{align*}
        \PP_{h_{A,b} \in H_{n,k}}\paren*{\dim{\ker{h}} \geq n-\delta} & \leq \paren*{\frac{1}{2^{n-\delta}}}^k \prod_{i=0}^{(\delta-1)} \frac{2^n-2^i}{2^{\delta}-2^i} = \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta}\paren*{\frac{1}{2^{n-\delta}}}^{\delta} \prod_{i=0}^{(\delta-1)} \frac{2^n-2^i}{2^{\delta}-2^i} \\
        & = \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \prod_{i=0}^{(\delta-1)} \frac{2^{\delta}-2^{i-n+\delta}}{2^{\delta}-2^i} \leq \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \prod_{i=0}^{(\delta-1)} \frac{2^{\delta}}{2^{\delta}-2^i}\\
        & = \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \prod_{i=0}^{(\delta-1)} \frac{2^{\delta-i}}{2^{\delta-i}-1} \leq \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \prod_{j=1}^{\infty} \frac{2^{j}}{2^{j}-1}\\
        & = \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \frac{1}{ \prod_{j=1}^{\infty} \paren*{1-2^{-j}} } \leq \paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} \frac{1}{1-\frac{1}{2}-\frac{1}{4}} \\
        & = 4\paren*{\frac{1}{2^{n-\delta}}}^{k-\delta} = 4 \paren*{\frac{1}{2^{n-k+c}}}^{c} = 4\paren*{\frac{1}{2^{n-k}}}^c \paren*{\frac{1}{2^c}}^c
    \end{align*}
    where the last inequality follows from Euler's pentagonal numbers theorem \cite{euler}.
    The final expression is less than \( \frac{1}{2^{c^{2}}} \) for \( c \geq 2 \) and \(n-k > 2\).
    \end{proof}
  
    Now we may describe the algorithm for solving unstructured search problem with known value \(k=1+\lceil \log_2{K} \rceil \) where \( K\) is the number of marked elements. 
    
    \begin{algorithm}
    \caption{Probabilistic algorithm for solving unstructured search with known \(k\)}
    
     \begin{algorithmic}[1]\label{multipoint}
         \captionsetup[algorithm]{name=MultiPoint}
         \Procedure{MultiPoint}{O, n, k} 
             \If{\(k \geq n-2\)}
                 \State \( x \gets \) element from \( \{0,1\}^n \) selected uniformly at random
                 \If{ \( x \) is marked}
                     \State \Return x
                 \EndIf
                 \State \Return null
             \EndIf
             \State \(h \gets\) random affine transformation from \( H_{n,k}\)
             \State \(d \gets \dim{\ker{h}} \) 
             \If{\( d \geq n-k+2\)}
                 \State \Return null
             \EndIf
             \State \(O_g \) is build as described in \Cref{oprim} using \(g\) from  \Cref{gauss-dziala}
             \State \Return \(\texttt{\texttt{SinglePoint}}(O_g, d)\) 
         \EndProcedure
  \end{algorithmic}  

    \end{algorithm}

    \multipoint*
    \begin{proof}
    To prove that \Cref{multipoint} finds a marked element with constant probability, let us see that if \(k \geq n-2\), then selecting a random element succeeds with probability at least \( \frac{1}{16} \).
    
    Otherwise from \Cref{valian-vazirani} with probability at least \(\frac{1}{8} \) we have that \(|K \cap \ker{h}| = 1 \). From \Cref{dimensionality}  with probability at least \( \frac{15}{16} \) we have that \( d < n-k+2 \). 
    Combining those facts we obtain that with probability at least \( \frac{1}{16} \) oracle \(O_g\) marks exactly one element and the number of qubits of its input does not exceed \( n-k+1 \). So \Cref{multipoint} succeeds with probability at least \( \frac{1}{16} \), as from \Cref{thm:main} we know that \(\texttt{SinglePoint}\) solves the unstructured problem with one marked element with certainty. 
    
    From \Cref{gauss-dziala} and \Cref{dekorator} we deduce that at most \(\calO(k)\)
     additional basic gates from circuit \(D_g\) depend on each qubit. So from \Cref{cor:average} we deduce that on average we use \(\calO(k)\) additional non-oracle basic gates per oracle query. There are \( \calO(2^{\frac{d}{2}}) = \calO(2^{\frac{n-k}{2}}) = \calO\paren*{\sqrt{\frac{N}{K}}}   \) oracle queries in \(\texttt{SinglePoint}\) procedure so  we need \( \calO(k2^{\frac{n-k}{2}}) =  \calO\paren*{\log{K}\sqrt{\frac{N}{K}}}\) non-oracle gates to implement it.    
    \end{proof}
    
    
    \begin{prop}\label{prob-amp}
    For any \(p\in (0,1)\) by repeating \Cref{multipoint} \(\calO(\log{\frac{1}{1 - p}})\) number of times we assure that we find a marked element with probability at least \(p\).
    \end{prop}
    \begin{proof}
    We may deduce that from the fact that all runs of this algorithm are independent and each finishes successfully with constant, non-zero probability.
    \end{proof}
    
    Let us for any probability \(p<1\) define an algorithm \( \texttt{MultiPointAmplified}(O, n, k, p) \) 
    which runs algorithm \(\texttt{MultiPoint}(O,n,k)\) minimal number of times to ensure probability of success higher than \(p\).
    
     
    
    \subsection{Unknown Number of Marked Elements}
    
    
    The technique presented next is similar to one used in \cite{inbook}, which finds element marked by an oracle \(O\) using on average \(\calO(2^{\frac{n-k}{2}})\) calls to oracle \(O\) and on average \(\calO(n2^{\frac{n-k}{2}})\) additional basic gates.
    We improve those result and propose the following algorithm that  finds marked element using 
        \( \calO( k2^{\frac{n-k}{2}})\) non-oracle gates in expectation and makes \( \calO( 2^{\frac{n-k}{2}})\) queries to oracle \(O\) also in expectation.
    
    
    
    \begin{algorithm}
    \caption{Probabilistic algorithm for solving unstructured search problem without an estimate of the number of marked elements}\label{alg:multipoint}
    
    \begin{algorithmic}[1]\label{multi-unknown}
        \Procedure{MultiPointUnknown}{O, n, p}
             \For{\(i \gets n+2\) to \(2\)}
                \For{\( j \gets n+2\) to \(i\)}
                    \State \(x \gets \texttt{MultiPointAmplified}(O, n, j, p)\)
                    \If{\( x \) is marked}
                    \State \Return x
                    \EndIf
                \EndFor
            \EndFor
        \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    
    
   
    Before we analyze \Cref{multi-unknown} we note an observation:
    
    
    \begin{observation}\label{mnoznik}
    For natural numbers \(x\) and \( m \), and any real number \(r\), such that \(x \leq m\) and \(r > 1\), we have \[
    \sum_{l=0}^{x}(m-l)r^{l/2} = (m-x)\sum_{l=0}^{x}r^{l/2} + \sum_{l=0}^{x}(x-l)r^{l/2} =
    (m-x)r^{x/2}\sum_{l=0}^{x}r^{(l-x)/2} + r^{x/2}\sum_{l=0}^{x}(x-l)r^{(l-x)/2} \leq\] \[ \leq (m-x)r^{x/2}\sum_{i=0}^{\infty}r^{-i/2} + r^{x/2}\sum_{i=0}^{\infty}ir^{-i/2}= C_1(m-x)r^{x/2}+C_2r^{x/2} \]
    Where \(C_1,C_2\) are positive constants which depend only on \(r\).
    \end{observation}
    
    
    \begin{observation}\label{mnoznik-2}
    For natural numbers \(x\) and \( m \), and any real number \(r\), such that \(x \leq m\) and \(r < 1\), we have 
    \[ \sum_{l=0}^{x}(m-l)r^{l/2}  \leq  Cm\] where \(C\) is a positive constant which depends only on \(r\).
    \end{observation}
    
    
    \begin{thm}
    For \( p \) satisfying \({2}(1-p)^2 < 1\) the \Cref{multi-unknown} finds marked element with probability at least \( 1-(1-p)^k \). Its expected number of oracle queries is \( \calO( \sqrt{\frac{N}{K}})\) and its expected number of non-oracle basic gates is \( \calO(\log{K} \sqrt{\frac{N}{K}})\), where \(N=2^n\) is the size of the search space and \(K\) is the number of elements marked by the oracle and \(k=1+\lceil \log_2{K} \rceil\).
    \end{thm}
    
    \begin{proof}
    In the complexity analysis we consider two phases of the \Cref{multi-unknown}. The first phase is when \( i > k\). During this phase we never run algorithm \texttt{MultiPointAmplified}(O, n, j,p) with \(j=k\), so let us assume that this algorithm never finds marked element in this phase.
    
    In the second phase i.e. for \( i < k\) in each inner loop we run the procedure {\texttt{MultiPointAmplified}(O, n, j, p)} with \(j=k\) once, so it during this loop we find marked element with probability at least \(p\). So the probability that outer loop proceeds to the next iteration is at most \(1-p\). 
    So overall bound on expected number of oracle queries of this algorithm is given below, we also note that all constants hidden under big \( \calO \) notation depend either only on \(p\) or are universal:
    
    \begin{align*}
    \calO &\paren*{\sum_{i=k+1}^{n+2} \sum_{j=i}^{n+2}2^{(n-j)/2} + \sum_{i=2}^{k}(1-p)^{k-i}\sum_{j=i}^{n+2}2^{(n-j)/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n} \sum_{j=i}^{n}2^{(n-j)/2} + \sum_{i=0}^{k}(1-p)^{k-i}\sum_{j=i}^{n}2^{(n-j)/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n} \sum_{l=0}^{n-i}2^{l/2} + \sum_{i=0}^{k}(1-p)^{k-i}\sum_{l=0}^{n-i}2^{l/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n} 2^{(n-i)/2} +\sum_{i=0}^{k}(1-p)^{k-i}2^{(n-i)/2}} = \\
      \calO&\paren*{ \sum_{s=0}^{n-k} 2^{s/2} + 2^{(n-k)/2}\sum_{s=0}^{k}(2(1-p)^{2})^{s/2}} = \calO \paren*{2^{(n-k)/2}}
    \end{align*}
    To estimate the second summand we use the fact that \(2(1-p)^2 < 1\).
    Using \Cref{mnoznik} and \Cref{mnoznik-2} we calculate the similar bound for the number of additional non-oracle basic gates, also take a note that hidden constants below depend only on \(p\) or are universal :
    
    \begin{align*}
    \calO &\paren*{\sum_{i=k+1}^{n+2} \sum_{j=i}^{n+2}j2^{(n-j)/2} + \sum_{i=2}^{k}(1-p)^{k-i}\sum_{j=i}^{n+2}j2^{(n-j)/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n} \sum_{j=i}^{n}j2^{(n-j)/2} + \sum_{i=0}^{k}(1-p)^{k-i}\sum_{j=i}^{n}j2^{(n-j)/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n} \sum_{l=0}^{n-i}(n-l)2^{l/2} + \sum_{i=0}^{k}(1-p)^{k-i}\sum_{l=0}^{n-i}(n-l)2^{l/2}} = \\
    \calO &\paren*{\sum_{i=k}^{n}i2^{(n-i)/2} +\sum_{i=0}^{k}i(1-p)^{k-i}2^{(n-i)/2}} = \\
      \calO&\paren*{ \sum_{s=0}^{n-k}(n-s)2^{s/2} + 2^{(n-k)/2}\sum_{s=0}^{k}(k-s)(2(1-p)^{2})^{s/2}} = \calO \paren*{k2^{(n-k)/2}}
    \end{align*}
    
    
    
    So the complexity of the algorithm does not change even if the number of elements is not a known beforehand. 
    To calculate the probability of successfully finding the marked element let's see that algorithm exits before the outer loop reaches the end of its range is when the marked element was found. From the above considerations we know that this probability is bounded from above by \((1-p)^k\).
    \end{proof} 
    

==> PartialUncompute.tex <==


\section{Partial uncompute}
\label{section:uncompute}

\subsection{Motivation and intuition}

The motivation for this section comes from the fact that many phase oracles mimic parallel
classical computation by the following pattern of operations.
\begin{enumerate}
    \item We perform a long series of operations that do not alter the original $n$ qubits (or alter them temporarily), but modify some number of ancilla qubits that were initially zero, usually by CCX gates.
    \item We perform a Z gate operation to flip the phase on the interesting states.
    \item We undo all the operations from step (1), not to hinder the amplitude intereference in the
    subsequent mixing operators.
\end{enumerate}
Step (3) offers the benefit of being able to reuse the (now cleared) ancilla qubits, but it is not the
main motivation of performing it.

If a mixing operators used only acts on a subset of qubits, maybe not all gates from step (1) interfere
with proper amiplitude interference? It turns out that very often it suffices to undo only a fraction of
gates. We will establish the proper language to express that in \cref{ss:uncompute-definitions}.

It turns out that the state that allows safe application of the mixing operator is much closer 
(in the metric of number of gates) to the state from after step (1) that to the base state with all
ancilla qubits zeroed. Our approach will initially compute all the ancilla qubits, perform all the
mixing ``close'' to this state, and finally uncompute the ancillas.

Intuitively, we shall follow the following new scheme.
\begin{enumerate}
    \item Compute all the ancilla qubits.
    \item For all mixing operators, perform the following.
    \begin{enumerate}
        \item Perform the phase flip.
        \item Undo the ancilla computation that would interfere with the upcoming mixing operator.
        \item Perform the mixing.
        \item Redo the computation from step 2(b).
    \end{enumerate}
    \item Uncompute all the ancilla qubits.
\end{enumerate}
The last step (2d) and step (3) could be even skipped, if the ancilla computation does not modify the 
original qubits. However we are not doing this optimization in the formal approach, as the benefits
are minimal.

Naturally, this is a very imprecise description. Full details are presented in  \cref{ss:uncompute-reducing}.

We are aware that many (if not all) of these operations are performed by modern quantum circuit
optimizers and preprocessors. The aim is to give structure to the process and understand how many
gates are guaranteed to be removed from the circuit.

\subsection{Definitions}
\label{ss:uncompute-definitions}

\begin{ddef}\label{def:uncomputable}
We will say that a phase oracle $O$ admits an \textit{uncomputable decomposition} $(O_u,O_p)$ if
$O=O_u^{\dagger}\circ O_p\circ O_u$. We call $O_u$ and $O_p$ the uncomputable part and the phase part,
respectively.
\end{ddef}

\begin{remark}Naturally, every phase oracle $O$ on $n$ qubits admits a trivial decomposition $(\id_n,O)$.
However, in practice, many real-life examples give more interesting decompositions.
\end{remark}

\begin{ddef}\label{def:depends}
Let $A_1,\dots,A_\ell$ be a chronologically ordered sequence of unitary matrices corresponding to the 
gates in a quantum circuit operating on $n$ qubits (ties being broken arbitrarily). We will define the
fact that \textit{$A_j$ depends on qubit $q_i$}, $i\in\{1,\dots,n\}$, by 
induction on $j\in\{1,\dots,\ell\}$.

We say that $A_j$ depends on $q_i$ if $A_j$ acts on $q_i$ or if there exist $i_0\in\{1,\dots,n\}$ and 
$j_0\in\{1,\dots,j-1\}$ such that the following hold.
\begin{itemize}
    \item $A_{j_0}$ depends on $q_i$.
    \item $A_{j_0}$ acts on $q_{i_0}$.
    \item $A_j$ acts on $q_{i_0}$.
\end{itemize}
\end{ddef}

\begin{ddef}
Let $O$ be a phase oracle on $n$ qubits, $\ell\in\mathbb N$,
$d:\{1,\dots,\ell\}\longrightarrow\mathcal P(\{q_1,\dots,q_n\})$,
and $U:\{1,\dots,\ell\}\ni j\longmapsto U_j\in U(n)$.
Assume that $U_j$ is an arbitrary unitary operator acting on the qubit set $d(j)$,
$j\in\{1,\dots,\ell\}$. We
define a \textit{generic oracle circuit} $V(\ell,d,U,O)$ by the following 
formula (the product is to be understood as right--to--left operator composition):
$$ 
V(\ell,d,U,O):=\prod_{j=1}^\ell
\left(U_j\circ O \right)
.
$$
\end{ddef}

\begin{remark}
Observe that $W_m$ from \cref{def:Wojter} is a generic oracle circuit.
\end{remark}

\begin{proof}
For $j\in\{1,\dots,m\}$ put $\ell_j:=(3^j-1)/2$ and define 
$d_j:\{1,\dots,\ell_j\}\longmapsto\mathcal P(\{1,\dots,k_1+\dots+k_j\})$ recursively
as follows:
$$
d_j(i):=
\begin{cases}
d_{j-1}(i)
,&
\quad
1\leq i\leq\ell_{j-1}
,
\\
\{k_1+\dots+k_{j-1}+1,\dots,k_1+\dots+k_j\}
,&
\quad
i=\ell_{j-1}+1
,
\\
d_{j-1}(2\ell_{j-1}+2-i)
,&
\quad
\ell_{j-1}+2\leq i\leq2\ell_{j-1}+1
,
\\
d_{j-1}(i-2\ell_{j-1}-1)
,&
\quad
2\ell_{j-1}+2\leq i\leq\ell_j
.
\end{cases}
$$
We then set $U_j$ to be the mixing operator $G_{|d_m(j)|}$ applied onto the qubits in the set 
$d_m(j)$, $j\in\ell_m$. Observe that $W_m=V(\ell_m,d_m,U,O)$.
\end{proof}

\subsection{Reducing the number of gates}
\label{ss:uncompute-reducing}

\begin{thm}\label{thm:subsets}
Let $(O_u,O_p)$ be an uncomputable decomposition of $O$ and let $D_u$, and $D_p$, be the total number 
of gates used in $O_u$, and $O_p$, respectively. Let $\overline D_s$ the number of gates 
within $O_u$ that depend on any of the qubits in $s$, $s\in\mathcal P(\{1,\dots,n\})$.

For a given generic oracle circuit $V(\ell,d,U,O)$ one can implement an equivalent circuit
$\widetilde V$ that uses a total of $2D_u+\ell D_p+2\sum_{j=1}^\ell\overline D_{d(j)}$ gates for oracle
queries. This results in no more than the following average number of gates per oracle query:
$$
D_p+2\frac{D_u}{\ell}+2\frac{\sum_{j=1}^\ell\overline D_{d(j)}}{\ell}.
$$
\end{thm}

\begin{proof}
Let $O_s$ (resp. $\widetilde O_s$) be the in-order composition of all gates in $O_u$ that depend
(resp. do not depend) on any of the qubits in $s$, $s\in\mathcal P(\{1,\dots,n\})$.

First, let us observe that, for a fixed $s\in\mathcal P(\{1,\dots,n\})$, every gate in $A\in O_j$
commutes with every
gate in $\widetilde O_s$ that originally appears later than $A$, as there are no common qubits that they 
act on. This implies that $O_u=O_s\circ\widetilde O_s$, $s\in\mathcal P(\{1,\dots,n\})$.

Similarly $U_j$ and $\widetilde O_{d(j)}$ commute,
as there are no common qubits that they act on, $j=1,\dots,\ell$.

We now proceed to apply these properties to $V(\ell,d,U,O)$ in order to obtain $\widetilde V$.
This will happen in the following five steps.
\begin{enumerate}
    \item Append an identity $O_u^\dagger\circ O_u$ operation to each factor of $V(\ell,d,U,O)$, see \cref{fig:uncompute-step-1}.
    \item Express $O_u$ (resp. $O_u^\dagger$) occuring next to $U_j$ as $O_{d(j)}\circ\widetilde O_{d(j)}$ (resp. $\widetilde O_{d(j)}^\dagger\circ O_{d(j)}^\dagger$ in the $j$th factor, $j\in\{1,\dots,\ell\}$, see \cref{fig:uncompute-step-2}.
    \item Swap $\widetilde O_{d(j)}$ and $U_j$ in the $j$th factor, $j\in\{1,\dots,\ell\}$, see \cref{fig:uncompute-step-3}.
    \item Remove the identity operation $\widetilde O_{d(j)}^\dagger\circ\widetilde O_{d(j)}$ in the $j$th factor, $j\in\{1,\dots,\ell\}$, see \cref{fig:uncompute-step-4}.
    \item Remove the identity operation $O_u\circ O_u^\dagger$ on the boundary between each two consecutive factors, see \cref{fig:uncompute-step-5}.
\end{enumerate}

    \begin{figure}[H]
            {\scriptsize
\begin{quantikz}[row sep=0.01cm, column sep=0.6cm]
           \lstick[3]{$d(j)$}     & \gate[wires=6][0.9cm]{O_u^\dagger} & \gate[6][0.9cm]{O_u}   & \gate[3]{U_j}           & \gate[6][0.9cm]{O_u^\dagger} & \gate[6][0.9cm]{O_p} & \gate[6][0.9cm]{O_u} &\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw                                & \qw                      & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw                                & \qw                      & \qw&\qw&\qw \\ 
            \lstick[3]{$\{1,\dots,n\}\setminus d(j)$}  & \ghost{W}                      & \qw                  &  \qw & \qw                      & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw                                & \qw                      & \qw&\qw&\qw \\ 
            \lstick{}          & \ghost{W}                      & \qw                  & \qw                                & \qw                      & \qw&\qw&\qw \\
        \end{quantikz}}
        \caption{Graphical representation of the $j$th factor after applying step (1).
        For simplicity we assumed that $d(j)$ consists of first $|d(j)|$ qubits.}
        \label{fig:uncompute-step-1}
    \end{figure}
    \begin{figure}[H]
            {\scriptsize
\begin{quantikz}[row sep=0.01cm, column sep=0.6cm]
           \lstick[3]{$d(j)$}     & \gate[wires=6][0.9cm]{O_u^\dagger} & \gate[6][0.9cm]{ O_{d(j)}}   & \qw & \gate[3]{U_j}          &\qw & \gate[6][0.9cm]{O_{d(j)}^\dagger} & \gate[6][0.9cm]{O_p} & \gate[6][0.9cm]{O_u} &\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw             &\qw                   & \qw                      &\qw& \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}                &\qw      & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\ 
            \lstick[3]{$\{1,\dots,n\}\setminus d(j)$}  & \ghost{W}                      &  \qw            &\gate[3][0.9cm]{\widetilde O_{d(j)}}      & \qw& \gate[3][0.9cm]{\widetilde O^\dagger_{d(j)}}& \qw                      & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}        &\qw              & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\ 
            \lstick{}          & \ghost{W}            &\qw          & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\
        \end{quantikz}}
        \caption{Graphical representation of the $j$th factor after applying step (2).
        For simplicity we assumed that $d(j)$ consists of first $|d(j)|$ qubits.}
        \label{fig:uncompute-step-2}
    \end{figure}

    \begin{figure}[H]
            {\scriptsize
\begin{quantikz}[row sep=0.01cm, column sep=0.6cm]
           \lstick[3]{$d(j)$}     & \gate[wires=6][0.9cm]{O_u^\dagger} & \gate[6][0.9cm]{ O_{d(j)}}   &  \gate[3]{U_j} &\qw         &\qw & \gate[6][0.9cm]{O_{d(j)}^\dagger} & \gate[6][0.9cm]{O_p} & \gate[6][0.9cm]{O_u} &\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw             &\qw                   & \qw                      &\qw& \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}                &\qw      & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\ 
            \lstick[3]{$\{1,\dots,n\}\setminus d(j)$}  & \ghost{W}                      &  \qw           &\qw &\gate[3][0.9cm]{\widetilde O_{d(j)}}      &  \gate[3][0.9cm]{\widetilde O^\dagger_{d(j)}}& \qw                      & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}        &\qw              & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\ 
            \lstick{}          & \ghost{W}            &\qw          & \qw                  & \qw             &\qw                   & \qw                      & \qw&\qw&\qw \\
        \end{quantikz}}
        \caption{Graphical representation of the $j$th factor after applying step (3).
        For simplicity we assumed that $d(j)$ consists of first $|d(j)|$ qubits.}
        \label{fig:uncompute-step-3}
    \end{figure}

    \begin{figure}[H]
            {\scriptsize
\begin{quantikz}[row sep=0.01cm, column sep=0.6cm]
           \lstick[3]{$d(j)$}     & \gate[wires=6][0.9cm]{O_u^\dagger} & \gate[6][0.9cm]{ O_{d(j)}}   &  \gate[3]{U_j} & \gate[6][0.9cm]{O_{d(j)}^\dagger} & \gate[6][0.9cm]{O_p} & \gate[6][0.9cm]{O_u} &\qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw             &\qw              & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}                &\qw      & \qw                  & \qw             &\qw           &\qw&\qw \\ 
            \lstick[3]{$\{1,\dots,n\}\setminus d(j)$}  & \ghost{W}                      &  \qw           &\qw & \qw                      & \qw&\qw&\qw \\
            \lstick{}          & \ghost{W}        &\qw              & \qw                  & \qw                                   & \qw&\qw&\qw \\ 
            \lstick{}          & \ghost{W}            &\qw          & \qw                  & \qw                                   & \qw&\qw&\qw \\
        \end{quantikz}}
        \caption{Graphical representation of the $j$th factor after applying step (4).
        For simplicity we assumed that $d(j)$ consists of first $|d(j)|$ qubits.}
        \label{fig:uncompute-step-4}
    \end{figure}

    \begin{figure}[H]
    {\scriptsize
        \begin{quantikz}[row sep=0.01cm, column sep=0.6cm]
           \lstick[3]{$d(j)$}     & \gate[6][0.9cm]{ O_{d(j)}}   &  \gate[3]{U_j} & \gate[6][0.9cm]{O_{d(j)}^\dagger} & \gate[6][0.9cm]{O_p} & \qw \\
            \lstick{}          & \ghost{W}                      & \qw                  & \qw             &\qw              & \qw\\
            \lstick{}          & \ghost{W}                &\qw      & \qw                  & \qw             &\qw            \\ 
            \lstick[3]{$\{1,\dots,n\}\setminus d(j)$}  & \ghost{W}                      &  \qw           &\qw & \qw                      & \qw \\
            \lstick{}          & \ghost{W}        &\qw              & \qw                  & \qw                                   & \qw \\ 
            \lstick{}          & \ghost{W}            &\qw          & \qw                  & \qw                                   & \qw \\
        \end{quantikz}
        }
        \caption{Graphical representation of the $j$th factor after applying step (5).
        For simplicity we assumed that $d(j)$ consists of first $|d(j)|$ qubits.
        Notice that this picture is only valid for $1<j<\ell$ as the first factor will retain $O^\dagger_u$, while the last one will retain $O_u$.}
        \label{fig:uncompute-step-5}
    \end{figure}

More concisely we put:
$$
\widetilde V:=O_u^\dagger
\circ
\prod_{j=1}^\ell
\left(
O_{d(j)}
\circ
U_j
\circ
O_{d(j)}^{\dagger}
\circ
O_p
\right)
\circ
O_u
.
$$
As discussed above $V(\ell,d,U,O)$ and $\widetilde V$ are equal as 
unitary operators. The desired gate count follows directly from the definition.
\end{proof}

\begin{corollary}\label{cor:weighted_average}
Let $(O_u,O_p)$ be an uncomputable decomposition of $O$ and let $D_u$, and $D_p$, be the total number 
of gates used in $O_u$, and $O_p$, respectively. 
Let $\overline D_j$ be the average number of gates within $O_u$ that depend on a single 
qubit from the $d(j)$, $j=1,\dots,\ell$. 
For a given generic oracle circuit $V(\ell,d,U,O)$ one can implement an equivalent circuit
$\widetilde V$
that uses no more than the following average number of gates per oracle query:
$$
D_p+2\frac{D_u+\sum_{j=1}^\ell|d(j)|\overline D_{d(j)}}{\ell}.
$$
\end{corollary}

\begin{proof}
This follows directly from \cref{thm:subsets} and the fact that the number of gates that depend on
any of the qubits from a given set is no greater that the sum of the numbers of gates that depend
on individual qubits from this set.
\end{proof}

\begin{corollary}\label{cor:average}
Let $(O_u,O_p)$ be an uncomputable decomposition of $O$ and let $D_u$, and $D_p$, be the total number 
of gates used in $O_u$, and $O_p$, respectively. 
Let $D$ be the average number of gates within $O_u$ that depend on a single 
qubit. 

For a given generic oracle circuit $V(\ell,d,U,O)$ one can implement an equivalent circuit
$\widetilde V$
that uses no more than the following average number of gates per oracle query:
$$
D_p+\frac{2D_u}{\ell}+2D\frac{\sum_{j=1}^\ell|d(j)|}{\ell}.
$$

In particular, one can implement a circuit equivalent to $W_m$ that uses an average of no more than
the following number of gates per oracle query:
$$
D_p+\frac{4D_u}{3^m-1}+4D\frac{\sum_{j=1}^mk_j3^{m-j}}{3^m-1}.
$$
Using the notation of \cref{thm:main}, this asymptotic average number of gates is
$\mathcal O(D_p+\log(1/\varepsilon)D)$.
\end{corollary}

\begin{proof}
Let $D_i$ be the number of gates within $O_u$ that depend on the $i$th qubit, $i\in\{1,\dots,n\}$.
Without loss of generality, we may assume that $(D_i)_{i=1}^n$ is non--decreasing. Similarly, without
loss of generality, we may assume that the weights $(|\{j\in\{1,\dots,\ell\}:i\in d(j)\}|/\ell)_{i=1}^n$ 
of subsequent qubits form a non--increasing sequence.
Such a weighted average of $D_i$s will
not be greater than their arithmetic mean. This completes the first part of the proof.

For the asymptotic result, recall from the proof of \cref{thm:main} that
$m=\Theta(\sqrt{n/\log(1/\varepsilon)}$ and we invoke the $W_m$ circuit $\mathcal O(2^{n/2}/3^m)$ times
with parameters $k_j\leq3\ceil{\log_2(1/\varepsilon)}j$, $j\in\{1,\dots,m\}$.
Additionally, observe that
$$
\sum_{j=1}^mj3^{m-j}=\sum_{j=1}^m\frac{3^{m-j+1}-1}2=\frac34(3^m-1)-\frac m2=\mathcal O(3^m-1).
$$
As each amplitude amplification step requires additional $\mathcal O(n+D_p+D_u)$ gates, we get that the asymptotic 
average number of gates is
$$
D_p+\mathcal O(D_u/3^m)+\log(1/\varepsilon)\mathcal O(D)+\mathcal O((n+D_p+D_u)/3^m)=\mathcal O(D_p+\log(1/\varepsilon)D).
$$
\end{proof}

\begin{corollary}\label{cor:ksat}
Let $K\in\mathbb N$ and consider all unique $K$--sat instances, each with $n$ variables and $c$ clauses. 
For each such an instance there exists a circuit equivalent to $W_m$ that uses an average of no more than 
the following number of gates per query:
$$
1+\frac{12Kc+8c-4}{3^m-1}
+
\frac{4Kc(4+\ceil{\log_2K}+\ceil{\log_2c})}n\cdot\frac{\sum_{j=1}^mk_j3^{m-j}}{3^m-1}.
$$
Using the notation of \cref{thm:main}, the asymptotic average per--oracle--query number of gates of a 
quantum circuit solving unique $K$--sat with certainty is
$\mathcal O(\log(1/\varepsilon)c\log(c)/n)$.
\end{corollary}

\begin{proof}
A straightforward implementation 
of the phase oracle $O$ consists of $D_u\leq 3Kc+2c-1$ gates (each being an X, a CX, or a CCX) in the 
uncomputable part and one Z gate ($D_p=1$) in the phase part.

More precisely, we introduce the following ancilla qubits and the gates to compute them:
\begin{enumerate}
    \item $c$ qubit groups of $K$ qubits corresponding to negation of all clause literals, each computed by one CX and at most one X,
    \item $c$ qubit groups of $K-1$ qubits corresponding to conjunctions of qubits from (1), each computed by one CCX. They are arranged into a binary tree, so that only $\ceil{\log_2K}$ gates depend on every qubit of (1).
    \item $c$ qubits corresponding to all clauses, each computed by one CX and one X from a top--level qubit of (2).
    \item $c-1$ qubits corresponding to conjunctions of qubits from (3), each computed by one CCX. Again, they are arranged into a binary tree, so that only $\ceil{\log_2c}$ gates depend on every qubit from (3).
\end{enumerate}

For a variable $v$ appearing in $c_v$ clauses, the 
number of gates depending on $v$ is at most $c_v(2+\ceil{\log_2K}+2+\ceil{\log_2c})$, so we get
the average $D\leq Kc(4+\ceil{\log_2K}+\ceil{\log_2c})/n$. By Corollary \ref{cor:average} we get both 
claims.
\end{proof}

\ksat*

\begin{proof}
This follows directly from \cref{thm:main} and \cref{cor:ksat}.
\end{proof}

==> backup.tex <==
\begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.4cm]
    	 	\lstick{ ${q}_{1}$  } & \ctrl{1} & \qw & \qw & \qw & \ctrl{1}  &\gate[1][1.8em]{T} & \qw  & \qw & \targ{} & \qw & \targ{} & \gate{R_1} & \targ{} & \qw & \control{} \qw & \gate{R_2} & \qw & \qw\\
    	 	\lstick{ ${q}_{3}$  } & \targ{} & \gate{T^\dag} & \targ{} & \gate[1][1.8em]{T} & \targ{} & \gate{T^\dag} & \ctrl{1} &\gate[1][1.8em]{T} & \ctrl{-1} & \targ{} & \ctrl{-1} & \qw & \ctrl{-1} & \targ{} & \ctrl{-1} & \qw & \qw & \qw\\
    	 	\lstick{ ${q}_{4}$  } & \qw & \qw & \ctrl{-1} & \qw & \qw &\qw &\targ{} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \gate{R_3} & \qw & \qw & \qw\\
    	 \end{quantikz}
        \caption{Simplified implementation of \(CCZ\) on qubits \(q_0, q_1, q_2\) in line topology, where $R_1 = U_2\left(\frac{5 \pi}{4},-\frac{5 \pi}{4}\right)$, $R_2 = U_2\left(0,-\frac{pi}{4}\right)$, $R_3 = U_3(0,-\frac{3 \pi}{4},-\pi)$}
        \label{fig:swap_simplified}
    \end{figure}
    
    
    
    

\section{Topology Aware Implementation}
\label{appendix:b}



By careful analysis of architecture of IBM Quantum Computers we reduce the number of \(CNOT\) gates in our circuits. 
IBM quantum computers allow for arbitrary \(1\)-qubit gates and for \(CNOT\) gates across links between qubits.
For example Vigo quantum computer is build as shown in \Cref{fig:figa_zmakiem}.

 


    \begin{figure}
        \centering
        \includegraphics[scale=0.5]{tgrup.eps}
        \caption{OP TOPOLOGIA 11/10}
        \label{fig:figa_zmakiem}
    \end{figure}



First one is to use qubit \(q_1\) as a target so that all \(2\)-qubit gates needed to perform Margolus gate can be run on neighbouring qubits.



To run a \(CCZ\) gate on qubits \(q_1, q_3, q_4\) with standard approach we would need to perform two swaps to let qubits \(q_1\) and \(q_4\) interact. Each swap is implemented with \(3\) entangling gate gates, resulting in cost of \(12\) \(CNOTs\) for each \(CCZ\) gate. 

    \begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.5cm]
    	 	\lstick{ ${q}_{0}$ } & \qw & \qw & \qw & \ctrl{2} & \qw & \qw & \qw & \qw & \qw & \ghost{O}\\
    	 	\lstick{ ${q}_{1}$ } & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ghost{O}\\
    	 	\lstick{ ${q}_{2}$ } & \gate{R_1} & \targ{} & \gate{R_1} & \targ{} & \gate{R_2} & \targ{} & \gate{R_2} & \qw & \qw & \ghost{O}\\
    	 \end{quantikz}
        \caption{Margolus gate, where $R_1 = U_3(\frac{\pi}{4},0,0)$ and $R_2 = U_3(-\frac{\pi}{4},0,0)$}
        \label{fig:swap}
    \end{figure}

  
    \begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.5cm]
    	 	\lstick{ ${q}_{1}$  } & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \gate[1][1.8em]{T} & \qw & \qw & \swap{} & \qw & \qw & \qw & \swap{} & \qw & \qw\\
    	 	\lstick{ ${q}_{3}$  } & \targ{} & \gate[1][1.8em]{T^\dag} & \targ{} & \gate[1][1.8em]{T} & \targ{} & \gate[1][1.8em]{T^\dag} & \targ{} & \gate[1][1.8em]{T} & \swap{-1} & \targ{} & \gate[1][1.8em]{T^\dag} & \targ{} & \swap{-1} & \qw & \qw\\
    	 	\lstick{ ${q}_{4}$  } & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \ctrl{-1} & \gate[1][1.8em]{T} & \ctrl{-1} & \qw & \qw & \qw\\
    	 \end{quantikz}
        \caption{Naïve implementation of \(CCZ\) on qubits \(q_0, q_1, q_2\) in line topology}
        \label{fig:swap}
    \end{figure}
    
It can be circumvented with the following more cost effective circuit. It requires only \(8\) \(CNOTs\). 
    
    
     \begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.6cm]
    	 	\lstick{ ${q}_{0}$ } & \gate{T^\dag} & \ctrl{1} & \qw & \ctrl{1} & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \qw\\
    	 	\lstick{ ${q}_{1}$ } & \gate{T^\dag} & \targ{} & \ctrl{1} & \targ{} & \ctrl{1} & \targ{} & \gate{Z} & \gate{T} & \ctrl{1} & \targ{} & \qw & \ctrl{1} & \qw & \qw\\
    	 	\lstick{ ${q}_{2}$ } & \gate{T^\dag} & \qw & \targ{} & \gate{T^\dag} & \targ{} & \gate{Z} & \gate{T} & \qw & \targ{} & \gate{Z} & \gate{T} & \targ{} & \qw & \qw\\
    	 \end{quantikz}
        \caption{Simplified implementation of \(CCZ\) on qubits \(q_0, q_1, q_2\) in line topology}
        \label{fig:swap_simplified_better}
    \end{figure}
    
    Implementation of diffusor on qubits \(q_3, q_4\) is straightforward and costs only \(1\) entangling gate. To implement diffusor on qubits \(q_0, q_2\) we would need to use two \(SWAP\) gates which would result in circuit with \(7\) entangling gate gates.
    
    \begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.4cm]
    	 	\lstick{ ${q}_{0}$  } & \gate{H} & \gate{X} & \swap{1} & \qw & \swap{1} & \gate{X} & \gate{H} & \qw & \qw\\
         	\lstick{  $\ket{0}$  } & \qw & \qw & \swap{-1} & \ctrl{1} & \swap{-1} & \qw & \qw & \qw & \qw\\
         	\lstick{ ${q}_{2}$  } & \gate{H} & \gate{X} & \qw & \control{}\qw & \qw & \gate{X} & \gate{H} & \qw & \qw\\
    	 \end{quantikz}
        \caption{Naïve diffusor on qubits \(q_0,q_2\) that are topologically separated by qubit \(q_1\)}
        \label{fig:diffusor_n}
    \end{figure}
    
    To reduce the amount of entangling gates we note that the circuit at \Cref{fig:diffusor} is equivalent to the circuit at \Cref{fig:diffusor_n} and requires only \(3\) two qubit gates. 
    
    \begin{figure}[ht]
        \begin{quantikz}[row sep=0.1cm, column sep=0.4cm]
    	 	\lstick{ ${q}_{0}$  } & \gate{H} & \gate{X} & \ctrl{1} & \qw & \ctrl{1} & \gate{X} & \gate{H} & \qw & \qw\\
         	\lstick{ $\ket{0}$  } & \qw & \qw & \targ{} & \ctrl{1} & \targ{} & \qw & \qw & \qw & \qw\\
         	\lstick{ ${q}_{2}$  } & \gate{H} & \gate{X} & \qw & \control{}\qw & \qw & \gate{X} & \gate{H} & \qw & \qw\\
    	 \end{quantikz}
        \caption{Diffusor on qubits \(q_0,q_2\) that are topologically separated by qubit \(q_1\)}
        \label{fig:diffusor}
    \end{figure}
   
    

==> dschewkher.tex <==
\appendix
\section{Analysis of the Tree circuit}
\label{appendix:a}

For the sake of completeness we include here a proof that the circuits \(D_n\) together with amplitude amplification \cite{ampamp} allow us to solve the unstructured search problem optimally. The notation we will work with here is analogous to the one used in section 3 of~\cite{prackum}.

\begin{lem}\label{lem:symmetry}
    Let \(m \in \mathbb{N}_{+}\) and \(\overline{k} \in \mathbb{N}_{+}^m\) be fixed, and let \(n = \sum_{j = 1}^{m} k_j\). Assume we are given a phase oracle \(O\) that operates on \(n\) qubits and marks a single vector of the standard computational basis, which we then use in the circuits \(D_j\).
    Then for any \(j \in \set{0, \dots, m}\) we have
    \[
        D_j O D_j = O \text{.}
    \]
\end{lem}
\begin{proof}
    We proceed by induction on \(j\). For \(j = 0\) the claim is trivial. For \(j > 0\) we expand \(D_j\) according to the recursive definition as follows
    \begin{align}
        D_j O D_j   &= D_{j - 1} \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} O D_{j - 1} O  D_{j - 1} \nonumber \\ & \quad \times \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} O D_{j - 1}  \nonumber \\
                    &= D_{j - 1} \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} O O \label{eqn:us1} \\ & \quad \times \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} O D_{j - 1} \nonumber \\
                    &= D_{j - 1} \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} \nonumber \\ & \quad \times \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}} O D_{j - 1} \nonumber \\
                    &= D_{j - 1}  O D_{j - 1} \nonumber \\
                    &= O \label{eqn:us2}
    \end{align}
    where in \cref{eqn:us1,eqn:us2} we used the inductive hypothesis.
\end{proof}

\begin{lem}\label{lem:recurrence}
    Let \(m \in \mathbb{N}_{+}\) and \(\overline{k} \in \mathbb{N}_{+}^m\) be fixed, and let \(n = \sum_{j = 1}^{m} k_j\). Assume we are given a phase oracle \(O\) that operates on \(n\) qubits and marks a single vector of the standard computational basis denoted \(\target\).
    Define the numbers 
    \[
        \beta_j = \bra{\target} \paren*{D_j \ket{u_1^j} \ket{\target_{j + 1}^{m}}}
    \]
    for \(j \in \set{0, \dots, m}\). Then \(\beta_j\) satisfy the recurrence
    % \[
    %     \beta_j = \begin{cases}
    %         1, & \ \text{ if }\ j = 0\\
    %         \frac{1}{2^{ (k_1 + \dots + k_j)/ 2}} \paren*{1 - \frac{2}{2^{k_j}}} + \frac{1}{2^{k_j / 2}} \paren*{2 - \frac{2}{2^{k_j / 2}}} \beta_{j - 1}, & \ \text{ if }\ j > 0 \text{.}
    %     \end{cases}
    % \]
    \begin{align*}
        \beta_0 & = 1 \\
        \beta_{j + 1} &= 2^{(k_1 + \dots + k_{j + 1}) / 2} \paren*{1 - \frac{2}{2^{k_{j + 1}}}}\\& \quad  + 2^{-k_{j + 1} / 2} \paren*{2 - \frac{2}{2^{k_{j + 1} / 2}}} \beta_j
    \end{align*}
\end{lem}
\begin{proof}
    By defintion of \(D_j\) we have \(\beta_0 = 1\) giving the base case.
    For \(j > 0\), we proceed to compute \(\beta_j\) by expanding the circuit \(D_j\) according to the recursive definition. We split the computation into stages as follows
    \begin{align*}
        \ket{w_1} &= D_{j-1} \paren*{\ket{u_1^j} \ket{\target_{j + 1}^{m}}}\\
        \ket{w_2} &= O \ket{w_1}\\
        \ket{w_3} &=  \paren*{\id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s}}\ket{w_2}\\
        \ket{w_4} &= D_{j - 1} \ket{w_3}
    \end{align*}
    where \(s = k_1 + \dots + k_j\).
    
    \begin{align}
        \ket{w_1}   &= D_{j - 1} \paren*{\frac{1}{2^{k_j / 2}}\ket{u_1^{j - 1}} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m}} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} D_{j - 1}\ket{u_1^{j - 1}} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m} \nonumber \\
        \ket{w_2}   &= O \paren*{\frac{1}{2^{k_j / 2}} D_{j - 1}\ket{u_1^{j - 1}} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m}} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} O D_{j - 1}\ket{u_1^{j - 1}} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \ket{\eta} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m} \nonumber \\
        \intertext{
        Where \(\ket{\eta}\) is some state in \(\paren*{\mathbb{C}^2}^{\otimes \paren*{k_1 + \dots + k_{j - 1}}}\). We can write so, as all diffusors within \(D_{j - 1}\) operate only on the prefix consisting of first \(k_1 + \dots + k_{j - 1}\) qubits, while \(O\) only changes relative phases.
        }
        \ket{w_3}   &= \id_{s - k_j} \otimes G_{k_j} \otimes \id_{n - s} \paren*{\frac{1}{2^{k_j / 2}} \ket{\eta} \ket{\target_j^m} + \ket{u_1^{j - 1}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^m}} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \ket{\eta} \paren*{G_{k_j} \ket{\target_j}} \ket{\target_{j + 1}^m} + \ket{u_1^{j - 1}} \paren*{G_{k_j}\ket{\overline{\target}_j}} \ket{\target_{j + 1}^m} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \ket{\eta} \paren*{\frac{2}{2^{k_j / 2}} \ket{u_j} - \ket{\target_j}} \ket{\target_{j + 1}^m} + \ket{u_1^{j - 1}} \paren*{\paren*{1 - \frac{2}{2^{k_j}}} \ket{u_j} + \frac{1}{2^{k_j / 2}} \ket{\target_j}} \ket{\target_{j + 1}^m} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \paren*{ \paren*{\frac{2}{2^{k_j}} - 1} \ket{\eta} + \paren*{2 - \frac{2}{2^{k_j}}} \ket{u_1^{j - 1}}} \ket{\target_j^m} + \paren*{\frac{2}{2^{k_j}} \ket{\eta} + \paren*{1 - \frac{2}{2^{k_j}}} \ket{u_1^{j - 1}}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^{m}} \nonumber \\
        \ket{w_4}   &= D_{j - 1} \ket{w_3} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \paren*{ \paren*{\frac{2}{2^{k_j}} - 1} O\ket{u_{1}^{j - 1}}\ket{\target_j^m} + \paren*{2 - \frac{2}{2^{k_j}}} D_{j - 1}\ket{u_1^{j - 1}} \ket{\target_{j}^m}} \nonumber\\ & \quad \quad + \paren*{\frac{2}{2^{k_j}} \ket{\eta} + \paren*{1 - \frac{2}{2^{k_j}}} \ket{u_1^{j - 1}}} \ket{\overline{\target}_j} \ket{\target_{j + 1}^{m}} \nonumber
    \end{align}
    Note that we used \cref{lem:symmetry} when applying \(D_{j - 1}\) in the first summand.
    Now we can plug \(\ket{w_4}\) into the expression defining \(\beta_j\). Observe that the second summand in final expression is orthogonal to \(\ket{\target}\), thus can be safely discarded. We obtain
    \begin{align}
        \beta_j     &= \bra{\target} \paren*{\frac{1}{2^{k_j / 2}} \paren*{ \paren*{\frac{2}{2^{k_j}} - 1} O\ket{u_{1}^{j - 1}}\ket{\target_j^m} + \paren*{2 - \frac{2}{2^{k_j}}} D_{j - 1}\ket{u_1^{j - 1}} \ket{\target_{j}^m}}} \nonumber \\
                    &= \frac{1}{2^{k_j / 2}} \paren*{ \paren*{1 - \frac{2}{2^{k_j}}} \frac{1}{2^{\paren*{s - k_j} / 2}} + \paren*{2 - \frac{2}{2^{k_j}}} \beta_{j - 1}} \nonumber \\
                    &= \frac{1}{2^{ \paren*{k_1 + \dots + k_j}/ 2}} \paren*{1 - \frac{2}{2^{k_j}}} + \frac{1}{2^{k_j / 2}} \paren*{2 - \frac{2}{2^{k_j / 2}}} \beta_{j - 1} \nonumber
    \end{align}
    concluding the proof.
\end{proof}
      \begin{thm}\label{thm:main}
            Fix any \(\varepsilon > 0\), and any \(N \in \mathbb{N}\) of the form $N = 2^n$. Suppose we are given a quantum oracle \(O\) operating on \(n\) qubits that marks exactly one element. Then there exists a quantum circuit \(\calA\) which uses the oracle \(O\) at most
            \(\paren*{1 + \varepsilon} \frac{\pi}{4} \sqrt{N}\) times
            and uses at most
            \(\calO \paren*{\log\paren*{\sfrac{1}{\varepsilon}} \sqrt{N}}\)
            non-oracle basic gates, which finds the element marked by \(O\) with certainty.
        \end{thm} 
\begin{proof}
    We first begin by choosing a particular sequence of sizes for diffusors in the circuit \(D_m\) -- namely \(k_j = (x + 1) \cdot j\) where \(x \in \mathbb{N}_{+}\) is some parameter, and let us assume that the number of qubits we work with is precisely \((x + 1) + (x + 1) \cdot 2 + \dots + (x + 1) \cdot m = (x + 1) m (m + 1) / 2\).
    From \cref{lem:recurrence}, we get that the amplitude the circuit \(D_m\) in the marked state is given by the following recurrence
    \[
        \beta_j = \begin{cases}
            1, & \ \text{ if }\ j = 0\\
            \frac{1}{2^{ (x + 1) j (j + 1) / 4}} \paren*{1 - \frac{2}{2^{(x + 1)j}}} + \frac{1}{2^{(x + 1) j / 2}} \paren*{2 - \frac{2}{2^{(x + 1) j / 2}}} \beta_{j - 1}, & \ \text{ if }\ j > 0 \text{.}
        \end{cases}
    \]
    To simplify the analysis of this recurrence, let us begin by substituting \(\gamma_j = \beta_j \cdot 2^{{(x + 1) j (j + 1)}/{4}} \cdot 2^{-j}\), which yields
    \[
        \gamma_j = \begin{cases}
            1, & \ \text{ if }\ j = 0\\
            \paren*{1 - 2 \cdot 2^{-(x + 1) j}} \cdot 2^{-j} + \paren*{1 - 2 ^{- (x + 1) j}} \gamma_{j - 1}, & \ \text{ if }\ j > 0 \text{.}
        \end{cases}
    \]
    We easily obtain the following inequality for \(j > 0\)
    \[
        \gamma_j \geq \paren*{1 - 2^{-xj}} \paren*{2^{-j} + \gamma_{j - 1}} \text{.}
    \]
    
    We may thus set
    \[
        \delta_j = \begin{cases}
            1, & \ \text{ if }\ j = 0\\
            \paren*{1 - 2^{-xj}} \paren*{2^{-j} + \delta_{j - 1}}, & \ \text{ if } \ j > 0
        \end{cases}
    \]
    and we easily obtain the inequality \(\gamma_j \geq \delta_j\). We can express the solution to this recurrence as a sum
    \[
        \delta_m = \sum_{j = 0}^{m - 1} 2^{j - m} \cdot \prod_{k = m - j}^{m} \paren*{1 - q^k} + \prod_{k = 1}^{m} \paren*{1 - q^k}
    \]
    where \(q = 2^{-x}\).
    
    For \(a \in \mathbb{N} \cup \set{\infty}\), let
    \[
        \calP(a) = \prod_{k = 1}^{a} \paren*{1 - q^k} \text{.}
    \]
    In terms of \(\calP(a)\), we can lower bound \(\delta_m\), as each term in our product is strictly less than 1, thus
    \[\delta_m \geq \sum_{j = 0}^{m - 1} 2^{-m + j} \calP(m) + \calP(m) = \sum_{j = 0}^{m} 2^{-j} \calP(m) = (2 - 2^{-m}) \calP(m) \geq (2 - 2^{-m}) \calP(\infty). \]
    We now need a lower bound on \(\calP(\infty)\), which we can obtain via Euler's Pentagonal Number Theorem \cite{euler}, which states that
    \[\calP(\infty) = \prod_{k=1}^{\infty} \left(1 - q^k \right)
    = 1 + \sum_{k = 1}^{\infty} (-1)^k \left(q^{{(3k -1) k}/{2}} + q^{{(3k + 1)k}/{2}} \right)\]
    from which, one can easily derive the inequality
    \[\calP(\infty) \geq 1 - q - q^2 \text{.}\]
    Combining these inequalities we get
    \begin{equation}
        \beta_m \geq (2 - 2^{-m}) \left(1 - 2^{-x} - 2^{-2x}\right) \cdot 2^{m} \cdot 2^{-{n}/{2}} \text{.}
        \label[ineq]{ineq:alp}
    \end{equation}
    By Amplitude Amplification \cite{ampamp}, we need 
    \[\floor*{\frac{\pi}{4 \theta_m}}\]
    iterations of the \(D_m\) circuit and its conjugate, where \(\theta_m = \arcsin{\beta_m}\)
    Consider the standard inequality for \(z \in (0, 1]\)
    \[\sin{z} \leq z\]
    which we can restate to
    \begin{equation}
        \frac{1}{\arcsin{z}} \leq \frac{1}{z}.
        \label[ineq]{ineq:arc}
    \end{equation}
    \Cref{ineq:alp,ineq:arc} together allow us to bound the number of iterations by
    \[\frac{\pi}{4} \cdot \frac{1}{2 - 2^{-m}} \cdot \frac{1}{1 - q - q^2} \cdot 2^{-m} \cdot 2^{n / 2}.\]
    Each \(D_m\) has exactly \(2^m - 1\) oracle calls, so one iteration has \(2^{m + 1} - 1\) oracle calls (tree, its conjugate and 1 extra call). Thus the number of oracle calls is at most
    \[\frac{\pi}{4} \cdot \frac{1}{2 - 2^{-m}} \cdot \frac{1}{1 - q - q^2} \cdot 2^{-m} \cdot 2^{{n}/{2}} \cdot \left(2^{m + 1} - 1\right) = \frac{\pi}{4}\cdot \frac{1}{1 - q - q^2}\cdot 2^{{n}/{2}}\]
    so we are only a factor of \(\frac{1}{1 - 2^{-x} - 2^{-2x}}\) away from optimal number of oracle calls.
    
    $D_m$ can be implemented with \(\calO(\sum_{k = 1}^{m} ky \cdot 2^{m - k})\) gates. So we get at most
    \[\calO\left( \left(\sum_{k = 1}^{m}kx \cdot 2^{m - k}\right) \cdot 2^{-m} \cdot 2^{{n}/{2}} \right) = \calO \left( \left(\sum_{k = 1}^{m}kx 2^{-k}\right) 2^{{n}/{2}} \right)\]
    non-oracle gates used by our algorithm. We use the following simple observation
    \[\sum_{k = 1}^{m} kx 2^{-k} \leq \sum_{k=1}^{\infty}kx 2^{-k} = 2x\]
    to get that the total number of nonoracle gates used by our algorithm is bounded by \(\calO \left( x \cdot 2^{{n}/{2}} \right)\).
    Thus, for any \(\varepsilon > 0\) that is sufficiently small, we obtain an algorithm that makes at most
    \[(1 + \varepsilon) \frac{\pi}{4} \cdot 2^{{n}/{2}}\]
    oracle calls, and uses at most
    \[\calO \left( \log \left( \varepsilon^{-1} \right) 2^{{n}/{2}} \right)\]
    non-oracle gates by setting \(x \in \Theta\paren*{\log\paren*{\varepsilon^{-1}}}\).
\end{proof}

==> lowerbound.tex <==
 \section{Optimality}
 \label{section:lowerbound}

In this section we  show the following lower bound for the number of oracle queries.



\begin{thm}\label{thm:lowerbound}
        Fix $p\in(0,1)$, \(n \in \mathbb{N}\) and \(N = 2^{n}\). Let $T=T(N,p)$ be the number of oracle queries in the optimal search algorithm that is needed to find the marked element with probability at least $p$. There exists a constant $C>0$, that possibly depends on $p$ but does not depend on $N$, such that for any $\eta>0$ and any algorithm \(\calA\) that uses at most  $\eta T$ additional elementary gates for finding marked element with probability $p$  needs to query oracle at least $\floor*{T+\sqrt N /2^{C\eta}}$ times.
        \end{thm}
    
        
        As a byproduct we  reprove the Zalka's estimation from \cite{zalka} (\cref{cor:Zalka}) and at the end of the section we shortly explain how the above theorem implies \cref{corollary:optimality}. 
  
   
  
    Let $m\geq n $ be the number of qubits which we use.
    Assume that we have at our disposal a phase oracle $O^y$ operating on $n$ qubits with the one marked element $y$. Any quantum algorithm that solves unstructured search problem  has the following form: we start with some initial quantum state $\ket{s}$ and apply the alternating sequence of oracle queries $O^y$ and unitary operators $U_1,\ldots,U_R$ (each of which acts on $m$ qubits). Thus as a result we get a state 
    \begin{equation*}
        \ket{t}=U_RO^yU_{R-1}O^y\ldots U_{1}O^y\ket{s}.
    \end{equation*}
     
     It is convenient to investigate the algorithm's behaviour for all possible $y\in\{0,1\}^n$ simultaneously. For this purpose we consider the following sphere and its subset.  Let $$S=\left\{z\in\left((\mathbb{C}^2)^{\otimes m}\right)^N:|z|=\sqrt N\right\}$$ and $$\hat S=\{(z_1,\ldots,z_n)\in S:z_1=\ldots=z_n\}.$$  
     
      Let $y_j$ for $j \in \set{1,\ldots,N}$ be a sequence of all elements of $\{0,1\}^n$. We use the   followings two actions of unitary group on the sphere $S$. For $U \in {\rm U}(2^{m})$ and $z$ in $S$ we put:
     \begin{equation*}
         Uz=(Uz_1,Uz_2,\ldots,Uz_N)
     \end{equation*}
     and
     \begin{equation*}
        O_Uz=(UO^{y_1}z_1,UO^{y_2}z_2,\ldots,UO^{y_N}z_N).
     \end{equation*}
     
    By straightforward calculations we get the following observation.
    
    \begin{observation}\label{observation:dwa} For $z$ in $\hat S$ we have \begin{equation*}
        |O_Uz-Uz|=2.
    \end{equation*}
    \end{observation}
    We  consider the following sequences of points on the sphere $S$.
    $$s_0=(\ket{s},\ldots,\ket{s})\hbox{ and }s_{i}= O_{U_R}\ldots O_{U_{i+1}}U_i\ldots U_1s_0.$$ Let us recall the inequality proved in \cite{inbook} (see also \cite{zalka}) which are crucial for our considerations.
    
  \begin{lem}\label{lem:crucial} If the algorithm  finds marked element with probability at least $p$ then
    \begin{equation}\label{crucialinequality}
         |s_R-s_0|^2\geq h(p) ,
      \end{equation}
      where $h$ is a function given by the formula $$h(p)=2N-2\sqrt N \sqrt p-2\sqrt N \sqrt{N-1}\sqrt{1-p}.$$
   \end{lem}
   
    The advantage of working on the sphere is  that the distance between points on the sphere $S$ is connected with the angle between them. For $a,b\in S$ let $\varphi_{a,b}$ be the angle between them i.e. 
    % $$\varphi_{a,b}=2\arcsin{\left(|a-b|/2\sqrt N\right)}\in[0,\pi].$$
    \[
        \varphi_{a,b} = 2 \arcsin \paren*{\frac{|{a - b}|}{2\sqrt{N}}} \in [0, \pi].
    \]
       Put 
$$\alpha=2\arcsin{\left(1/\sqrt N\right)}.$$ Now let us consider distances between elements of sequence $s_i$.

\begin{observation}  For $i \in \set{0,\ldots,R-1}$ we have \begin{equation*}
      |s_i-s_{i+1}|=2  \ \hbox{ and } \ \varphi_{s_is_{i+1}}=\alpha. 
  \end{equation*}
    \end{observation}
 
 
  \begin{proof}
  By \cref{observation:dwa} we have 
  \begin{equation*}
      |s_i-s_{i+1}|=|O_Uz-Uz|=2, 
  \end{equation*}
  where $U=U_{i+1}$ and $z=U_i\ldots U_1s_0$.
\end{proof}

\begin{observation}\label{observation:niertrdlakat} The following inequality holds  \begin{equation*}
    \varphi_{s_0s_{R}}\leq R\alpha. 
  \end{equation*}
    \end{observation}
 
  \begin{proof}
 The Observation holds by the previous Observation and the triangle inequality.
\end{proof}


      If we look  at Grover's  algorithm we can notice the following facts.
    
      \begin{observation} \label{observation:Grover-rownosc} In case of Grover's algorithm we have the equality in (\ref{crucialinequality}) for $R\leq(\frac{\pi}{\alpha}-1)/2$.
    \end{observation}
    
      \begin{observation} In case of Grover's algorithm  all points $s_0,\ldots,s_P$ lie on the great circle of the sphere $S$.
    \end{observation}
     
      
     
   
 
 
\begin{lem}
 For a given $R\leq(\frac{2\pi}{\alpha}-1)/2$ the expression $|s_R-s_0|$ is maximised by Grover's algorithm.\end{lem}

\begin{proof}
Since in the case of Grover's algorithm points $s_0,\ldots,s_R$ lie on the great circle we get $\varphi_{s_0s_{R}}=R\alpha$ and thus the distance between $s_0$ and $s_R$ is maximised.
\end{proof}

Let us here recall the result of Zalka.
By above Lemma, \cref{observation:Grover-rownosc} and \cref{lem:crucial}  we get the following.
\begin{corollary}[Zalka's lower bound for search algorithm]\label{cor:Zalka}
 Let $R\leq(\frac{2\pi}{\alpha}-1)/2$. The Grover's algorithm that makes $R$ oracle queries gives maximal probability of measuring marked element among all quantum circuits that solve unstructured quantum search problem using at most $R$ queries.
\end{corollary}
Note that for large $N$ the number $\frac{\pi}{2\alpha}$ is close to $\frac{\pi}{4}\sqrt N$.

Now let us see what happens after two steps of the algorithm. Put $d_K=16(K-1)/K$ for $K\geq1$.

\begin{observation}\label{observation:dwakroki} If $z\in\hat S$, then $|O_{Id}O_Uz-Uz|^2\leq d_N$. In particular for $i \in \set{0,\ldots,R-2}$ we have \begin{equation*}
      |s_i-s_{i+2}|^2\leq d_N . 
  \end{equation*}
    \end{observation}


  \begin{proof}
  It is the direct consequence of \cref{observation:niertrdlakat} for $R=2$. 
\end{proof}

The key observation for  our lower bound is better estimation for unitary operators that act on bounded number of qubits. From this point of view we consider that each oracle query can be performed on arbitrary qubits in arbitrary order (or we can think that we just add SWAP gates). To stress this we use here the symbols $O$ and $O'$ for oracle operators.

 


   \begin{lem} \label{lem:technical}Let $z=(\ket{z},\ldots,\ket{z})\in\hat S$. If $U$  acts at most on $k$ qubits, then $|O'_{Id}O_Uz-Uz|^2\leq d_{K^2}$ where $K=2^k$.
   \end{lem}
      
    
 \begin{proof}   Let $A_U$ be the set of $k$ qubits on which $U$  acts. Oracle $O$ acts on qubits $Q_1,\ldots,Q_n$ and $O'$ on $Q_1',\ldots,Q_n'$ (here of course the order of qubits is important). We can choose a set of indices $J=\{j_1,\ldots,j
 _a\}$ such that $a\leq 2k$ and for $Q\in A_U$ if $O$ acts on $Q$ then $Q\in\{Q_{j_1},\ldots,Q_{j_a}\}$ and similarly if $Q\in\{Q_1',\ldots,Q_n'\}$ then $Q\in\{Q_{j_1}',\ldots,Q_{j_a}'\}$.
 Without loss of generality we can assume that $J= \{n+1-a,\ldots,n\}$. Put $$B=A_U\cup\{Q_{n+1-a},\ldots,Q_{n}\}\cup\{Q_{n+1-a}',\ldots,Q_{n}'\}.$$
 Let $B'$ be a set of others qubits and we assume that it is prefix of the set of all qubits.
%  We can see that $|B|<5k$.
 
 
 
 
 Let us fix for a moment $y=(y_1,\ldots,y_n)$. Let $q=(y_1,\ldots,y_{n-a})\in\{0,1\}^{n-a}$ and $r=(y_{n-a+1},\ldots,y_{n})\in\{0,1\}^{a}$. Sometimes we write $qr$ in place of $y$. We can write $\ket{z}$ as:
  \begin{equation*}
 \ket{z} =\sum_{\ket{x}\in\mathcal{B}'}\alpha_{x}\ket{x}\ket{S_{x}},
 \end{equation*}

 
 where $\mathcal{B'}$ is a computational basis in the space related to qubits from $B'$, $ \alpha_{x}$  are complex numbers and $\ket{S_{x}} $ are states  in the space related to qubits in $B$. It is clear that
 \begin{equation*}
 \sum_{\ket{x}\in\mathcal{B}'}|\alpha_{x}|^2=1.
 \end{equation*}
 We group elements of $\mathcal{B}'$ into four disjoint sets. Let $\mathcal{B}_1^q$ be the set of all  $\ket x$  that agree with $p_j$ on qubits $Q_j$ and $Q_j'$ for all $j\leq n-a$. Let $\mathcal{B}_2^q$ (respectively $\mathcal{B}_3^q$) be the set of all $\ket x$  that agree with $p_j$ on qubits $Q_j$ (respectively $Q_j'$) for all $j\leq n-a$ but differes on at least one qubit $Q_j'$ (respectively $Q_j$) for some $j\leq n-a$. And finally we put $\mathcal{B}_4^q=\mathcal{B}'\setminus\left(\mathcal{B}_1^q\cup\mathcal{B}_2^q\cup\mathcal{B}_3^q\right)$. Now we have \begin{equation*}
     \ket{z}=\sum_{i=1}^4\ket{z_i^q}
 \end{equation*}
 where \begin{equation*}\ket{z_i^q}=\sum_{\ket{x}\in\mathcal{B}_i^q}\alpha_{x}\ket{x}\ket{S_{x}}.\end{equation*}
 We have 
 \begin{align*}
     U\ket{z_i^q} & = \sum_{\ket{x}\in\mathcal{B}_i^q}\alpha_{x}\ket{x}U\ket{S_{x}},\\
     O'^{y} UO^y\ket{z_1^q} & = \sum_{\ket{x}\in\mathcal{B}_1^q}\alpha_{x}\ket{x}O'^rUO^r\ket{S_{x}}\\
     O'^{y} UO^y\ket{z_2^q} &  = \sum_{\ket{x}\in\mathcal{B}_2^q}\alpha_{x}\ket{x}UO^r\ket{S_{x}}\\
     O'^{y} UO^y\ket{z_3^q} & = \sum_{\ket{x}\in\mathcal{B}_3^q}\alpha_{x}\ket{x}O'^rU\ket{S_{x}}\\
     O'^{y} UO^y\ket{z_1^q} & = U\ket{z_1^q}
 \end{align*}
  where $O^r$ (and respectively $O'^r$) are oracles on $a$ qubits that mark element of the computational basis if for $k>n-a$ on $Q_{k}$ (respectively on $Q_{k}'$) this element is $p_{k}$.  We get
   \begin{equation*}
|O'^{y} UO^{y}\ket{z}-U\ket{z}|^2=\sum_{\ket{x}\in\mathcal{B}_1^q}|\alpha_{x}|^2|(U-O'^rUO^r)\ket{S_{x}}|^2+\sum_{\ket{x}\in\mathcal{B}_2^q}|\alpha_{x}|^2|(1-O^r)\ket{S_{x}}|^2+\sum_{\ket{x}\in\mathcal{B}_3^q}|\alpha_{x}|^2|(1-O'^r)U\ket{S_{x}}|^2\end{equation*}
 
  Now we are ready to sum up above expression with respect to $r$. For fixed $q$ we get
 
 \begin{equation*}
\sum_r |O'^{qr} UO^{qr}\ket{z}-U\ket{z}|^2\end{equation*}
 \begin{equation*} =\sum_{\ket{x}\in\mathcal{B}_1^q}|\alpha_{x}|^2|\sum_r(O'^rUO^r-U)\ket{S_x}|^2+4\sum_{\ket{x}\in\mathcal{B}_2^q}|\alpha_{x}|^2+4\sum_{\ket{x}\in\mathcal{B}_3^q}|\alpha_{x}|^2
 \end{equation*}
  \begin{equation*} \leq d_{2^a}\sum_{\ket{x}\in\mathcal{B}_1^q}|\alpha_{x}|^2+4\sum_{\ket{x}\in\mathcal{B}_2^q\cup\mathcal{B}_3^q}|\alpha_{x}|^2
  \end{equation*}
   \begin{equation*} \leq d_{K^2}/2\left(\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_2^q}|\alpha_{x}|^2+\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_3^q}|\alpha_{x}|^2\right).
  \end{equation*}
  The  inequality in third line holds by applying \cref{observation:dwakroki} in case of $R=2k$. 
  
   The next step is to estimate the sum above with respect to $q$. We have  
  \begin{equation*}
      \ket{z}=\sum_q\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_2^q}\alpha_{x}\ket{x}\ket{S_{x}} =\sum_q\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_3^q}\alpha_{x}\ket{x}\ket{S_{x}} 
  \end{equation*}
  and thus
  \begin{equation*}
      \sum_q\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_2^q}|\alpha_{x}|^2 =\sum_q\sum_{\ket{x}\in\mathcal{B}_1^q\cup\mathcal{B}_3^q}|\alpha_{x}|^2 =1.
  \end{equation*}
  
  Finally we can conclude
   \begin{equation*}
|O'_{Id}O_Uz-Uz|^2=\sum_y |O'^{y} UO^y\ket{z}-U\ket{z}|^2=\sum_q\sum_r |O'^{qr} UO^{qr}\ket{z}-U\ket{z}|^2\leq d_{K^2}.\end{equation*}
 
 
 \end{proof}
 

  
 

   
     
     \begin{proof}[\bf proof of \cref{thm:lowerbound}
     ]
    By \cref{observation:niertrdlakat} and \cref{lem:technical}  for $i \in \set{0,\dots,R-2}$ we have \begin{equation*}        \varphi_{s_is_{i+2}}\leq 2\alpha
    \end{equation*}
     and if $U_{i+1}$ acts on $k\leq n/4$ qubits
     \begin{equation*}        \varphi_{s_is_{i+2}}\leq \arcsin\left((4-(d_N-d_{K^2}))/\sqrt{N}\right)\leq \alpha\left(2-\frac{D}{K^2}\right)
    \end{equation*}
    where the constant $D$ (as well as constants $D'$ and $D''$ below)  does not depend on $N$ and $K$. From the triangle inequality
     we can estimate:
       \begin{equation*}
          \varphi_{s_Rs_0} \leq\alpha+\sum_{t\in\{l\in\mathbb{N}:2l+2\leq R\}}\varphi_{s_{2t},s_{2t+2}}.
      \end{equation*}
      
     We can choose $k$ (proportional to $\eta$) such that at least half of operators $U_{2t+1}$ act at most on $k$ qubits and now we have 
    
     \begin{equation*}
          \varphi_{s_Rs_0} \leq(R+1)\alpha-\frac{D'R}{K^2}\alpha\leq\alpha R(1-2^{-D''\eta})+\alpha.
      \end{equation*}
      On the other hand by \cref{lem:crucial} and
     \cref{observation:Grover-rownosc} we have 
       \begin{equation*}
          \varphi_{s_Rs_0} \geq(T-1)\alpha
      \end{equation*}
     and thus
     \begin{equation*}
          R\geq T-2+2^{-D''\eta}/\alpha.
      \end{equation*}
Let us choose $N_0$ such that $2^{-D''\eta}/\alpha  \geq 3$. There   is constant $C>0$ such that 
\begin{equation*}
 \sqrt N /2^{C\eta}\leq   2^{-D''\eta}/\alpha \hbox{ for } N\geq N_0
\end{equation*}
and
\begin{equation*}
 \sqrt N /2^{C\eta}<   1 \hbox{ for } N< N_0.
\end{equation*}
Since $R\geq T$ the theorem holds with such $C$.
          \end{proof}
          
 \begin{proof}[proof of \cref{corollary:optimality}]  

 One can see that any algorithm needs more than $\frac{\pi}{4}\sqrt{N}-1$ steps to find the marked element with certainty (compare \cref{cor:Zalka}).   Using \cref{thm:lowerbound} we get the result for $\delta=1/C$ and for $n$ large enough. If necessary, we may decrease $\delta$ so that \( \delta\log\paren*{\sfrac{1}{\varepsilon}} \sqrt{N}<1\) for smaller values of $n$.\end{proof}

 \begin{remark}Note that we do not allow  measurements before the end of the algorithm. It is not clear for authors how measurements performed inside circuit can reduce the expected number of oracle queries, in particular how Zalka’s
results about optimality of Grover’s algorithm translate to this more general class of quantum algorithms with the
measurements during the algorithm. Example of measurements speeding up quantum procedures can be found in
section 4 of \cite{inbook} or in the last section of this paper.
\end{remark}

==> text_circuit.tex <==
% \documentclass[border=6pt]{standalone}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}

% \usepackage{qcircuit}

% \title{Drawing Circuits with qcircuit}

% % \begin{document}

% \Qcircuit @C=1em @R=.7em {
% & \ctrl{2} & \targ & \gate{U} & \qw \\
% & \qw & \ctrl{-1} & \qw & \qw \\
% & \targ & \ctrl{-1} & \ctrl{-2} & \qw \\
% & \qw & \ctrl{-1} & \qw & \qw
% }

% \end{document}


==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
